Tweaking Metasploit to Evade Encrypted C2 Traffic Detection

Command and Control (C2) communication is a key component of any structured cyber-attack. As such, security operations actively try to detect this type of communication in their networks. This poses a problem for legitimate pentesters that try to remain undetected, since commonly used pentesting tools, such as Metasploit, generate constant traffic patterns that are easily distinguishable from regular web traffic. In this paper we start with these identifiable patterns in Metasploit's C2 traffic and show that a machine learning-based detector is able to detect the presence of such traffic with high accuracy, even when encrypted. We then outline and implement a set of modifications to the Metasploit framework in order to decrease the detection rates of such classifier. To evaluate the performance of these modifications, we use two threat models with increasing awareness of these modifications. We look at the detection evasion performance and at the byte count and runtime overhead of the modifications. Our results show that for the second, increased-awareness threat model the framework-side traffic modifications yield a better detection avoidance rate (90%) than payload-side only modifications (50%). We also show that although the modifications use up to 3 times more TLS payload bytes than the original, the runtime does not significantly change and the total number of bytes (including TLS payload) reduces.

==> detectionAvoidance.tex <==
% !TeX root = main.tex
\section{Detection avoidance:}

\begin{itemize}
    \item Threat model 1:
    \begin{itemize}
        \item Static Stuffing (in Payload and/or Framework);
        \item N Req/TCP (with/without Static Stuffing);
    \end{itemize}
    \item Threat model 2:
    \begin{itemize}
        \item N Req/TCP (with/without Static Stuffing) - Para mostrar que falha;
        \item Adv Stuffing with N Req/TCP based on Adv (Payload-Framework sync
            and no syn);
    \end{itemize}
\end{itemize}

